BEV-LaneDet: a Simple and Effective 3D Lane Detection Baseline

3D lane detection which plays a crucial role in vehicle routing, has recently been a rapidly developing topic in autonomous driving. Previous works struggle with practicality due to their complicated spatial transformations and inflexible representations of 3D lanes. Faced with the issues, our work proposes an efficient and robust monocular 3D lane detection called BEV-LaneDet with three main contributions. First, we introduce the Virtual Camera that unifies the in/extrinsic parameters of cameras mounted on different vehicles to guarantee the consistency of the spatial relationship among cameras. It can effectively promote the learning procedure due to the unified visual space. We secondly propose a simple but efficient 3D lane representation called Key-Points Representation. This module is more suitable to represent the complicated and diverse 3D lane structures. At last, we present a light-weight and chip-friendly spatial transformation module named Spatial Transformation Pyramid to transform multiscale front-view features into BEV features. Experimental results demonstrate that our work outperforms the state-of-the-art approaches in terms of F-Score, being 10.6% higher on the OpenLane dataset and 5.9% higher on the Apollo 3D synthetic dataset, with a speed of 185 FPS. The source code will released at https://github.com/gigo-team/bev_lane_det.

==> chapter/introducion_backup.tex <==
%
%\textbf{2D Lane Detection.}
 As one of the fundamental guarantees for autonomous driving, lane detection has recently received much attention from researchers. Robust lane detection in real-time is one of the foundations for advanced autonomous driving, which can provide substantial amounts of useful information for Autonomous Driving Systems (ADS), vehicle self-control, localization, and map construction.
\begin{figure}[ht]
    \centering
    % \begin{minipage}[c]{0.62\textwidth}
      \includegraphics[width=.5\textwidth]{figure/struct.pdf}
    % \end{minipage} ~ % HY: controls lateral space
    % \begin{minipage}[c]{0.34\textwidth}
    %\vspace{-.2cm}
      \caption{\textbf{End-to-end framework illustrated.} The original image in bottom-right is transformed to an input image by \textit{Virtual Camera} module. The input image is then encoded  to front-view features by the backbone. Multiscale features from backbone are put into \textit{Spatial Transformation Pyramid} (STP) to obtain BEV features. Given the BEV features, the 3D Head called \textit{Key-Points Representation} generates BEV output and Z, the height of BEV lanes. At last, with the BEV output and Z, we can obtain 3D lanes.}
    \label{fig:struct}
\end{figure}

2D lane detection methods have demonstrated remarkable performances in 2D image space \cite{cordts2016cityscapes,pan2018spatial,neven2018towards,liu2021condlanenet}. Moreover, the output of the 2D lane detection methods are usually projected to the flat ground plane by Inverse Perspective Transformation (IPM) with the camera intrinsic and extrinsic parameters, and then curve fitting is performed to obtain the BEV lanes based on the vehicle-ego coordinate system. However, the pipeline might cause other problems in the actual driving process \cite{bai2018deep,neven2018towards} for challenging situations like uphill and downhill.

In order to overcome these problems and enhance the lane detection in autonomous driving to an industrial-grade product application, more recent methods \cite{garnett20193d,efrat20203d,guo2020gen,li2022reconstruct,chen2022persformer} have started to focus on the more complicated 3D lane perception domain. There are two significant challenges in 3D lane detection: an efficient spatial transformation module to obtain BEV features and a robust representation for 3D lane structures. The acquisition of BEV features is heavily dependent on camera in/extrinsic parameters, and previous methods have chosen to incorporate camera in/extrinsic parameters into the network to obtain BEV features. These methods increase the learning cost of the network. Moreover, unlike obstacles on the road, lane structures are slender and diverse. These methods \cite{garnett20193d, guo2020gen, chen2022persformer} carefully design the 3D anchor representation for lane structure with strong priors. However, they lack sufficient flexibility in some specific scenarios. The detailed visualization can be found in Appendix. Moreover, the anchor-free method \cite{efrat20203d} propose a 3D lane representation based on a hypothesis that a line segment in each predefined tile is straight. This representation is complicated and unreasonable.

Towards the issues, we introduce BEV-LaneDet, an efficient and real-time pipeline that achieves 3D lane detection from a single image, as shown in Figure \ref{fig:struct}. Different from the methods of incorporating camera in/extrinsic parameters into the network to get BEV features, we establish a \textit{Virtual Camera}, which is applied to images directly. The module unifies the in/extrinsic parameters of front-facing cameras in different vehicles by the homography method\cite{homographies} based on BEV. This module guarantees the consistency of the spatial relationship of front-facing cameras in different vehicles and reduces variance in data distribution. It reduces the learning cost of the network. We also propose a \textit{Key-Points Representation} as our 3D lane representation. We demonstrate that it is a simple but effective module to represent 3D lanes and is more expandable for complicated lane structures in some special scenarios. Moreover, the cost of computation and the chip's friendliness are also crucial factors in autonomous driving. Therefore, a light-weight and easy-to-deploy spatial transformation module based on MLP is our preference. Meanwhile, inspired by FPN\cite{lin2017feature}, we present the \textit{Spatial Transformation Pyramid}, which transforms multiscale front-view features to BEV and provides robust BEV features for 3D lane detection. In our experiments, we perform extensive studies to confirm that our BEV-LaneDet significantly outperforms the previous state-of-the-art PersFormer \cite{chen2022persformer} in terms of F-Score, by up to nearly 10.6\% with respect to the OpenLane real-world test set \cite{chen2022persformer}  and 4.0\% F-Score on the Apollo simulation test set \cite{guo2020gen} with a speed of 185 FPS.



\textbf{In summary, our main contributions are three-fold:} \textbf{1)} \textit{Virtual Camera}, a novel preprocessing module to unify the in/extrinsic parameters of cameras, ensuring data distribution consistency. \textbf{2)} \textit{Key-Points Representation}, a simple but effective representation of 3D lanes. \textbf{3)} \textit{Spatial Transformation Pyramid}, a light-weight and easy-to-deploy architecture based on MLP to realize transformation from multiscale front-view features to BEV. Experiments demonstrate that our BEV-LaneDet achieves state-of-the-art performance compared to other 3D lane detection algorithms.
%, and use Transformers to get BEV features which we describe below. 

==> table/speed.tex <==
\begin{table}[h]
\caption{The complexity and FPS on V-100}
\centering
\label{table: speed}
\scalebox{0.8}{
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Method} & \textbf{F-Score/OpenLane} & \textbf{GFLOPs} & \textbf{TensorRT} & \textbf{PyTorch} \\ \midrule
Gen-LaneNet     & 29.7             & 34                & --          & 54FPS \\
PersFormer      & 47.8             & 143                & --           & 21FPS \\
Ours            & 58.4             & 53                & 185FPS          & 102FPS \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/table_ablation.tex <==
\begin{table*}[t]
\centering
\caption{Ablation studies on the Openlane. VC: \textit{Virtual Camera}; STP: \textit{Spatial Transform Pyramid}; Cell size 0.5: the cell size of KPR is 0.5; 2D: front-view auxiliary head.}
\label{table: ablation}
\label{table: head}
\begin{tabular}{@{}lllllll@{}}
\toprule
\textbf{Method} & \textbf{F-Score} & \textbf{X error near} & \textbf{X error far} & \textbf{Z error near} & \textbf{Z error far} & \textbf{FPS} \\ \midrule
Baseline(ResNet34)   & 48.7             & 0.376                 & 0.791                & 0.265                 & 0.713                & -               \\
+ VC     & 53.3             & 0.324                 & 0.695                & 0.330                 & 0.705                & -               \\
+ 2D             & 54.5             & 0.338                 & 0.689                & 0.258                 & \textbf{0.614}                & -               \\
+ STP                & 55.7             & 0.321                 & 0.701                & 0.253                 & 0.624                & -               \\
Cell size 0.5 (BEV-LaneDet) & \textbf{58.4}             & \textbf{0.309}                 & \textbf{0.659}                & \textbf{0.244}                 & 0.631                & 185               \\
BEV-LaneDet (ResNet18) & 57.8             & 0.318                 & 0.705                & 0.245                 & 0.629                & 272               \\ \bottomrule
\end{tabular}
\end{table*}

==> table/table_ablation_rebuttal.tex <==
% \begin{table}[]
% \caption{Ablation studies on the Openlane of our three modules. VC: \textit{Virtual Camera}; STP: \textit{Spatial Transform Pyramid}; KPR: \textit{Key-Points Representation}}
% \centering
% \label{table: ablation_rebuttal}
% \begin{tabular}{@{}lll|l@{}}
% \toprule
% \textbf{VC} & \textbf{STP} & \textbf{KPR} & \textbf{F-Score} \\ \midrule
%             &              &              &                  \\
% \checkmark           &              &              &                  \\
%             & \checkmark            &              &                  \\
%             &              & \checkmark            &                  \\
%             & \checkmark            & \checkmark            &                  \\
% \checkmark           &              & \checkmark            &                  \\
% \checkmark           & \checkmark            & \checkmark            &                  \\ \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[]
\caption{Ablation studies on the Openlane. VC: \textit{Virtual Camera}; STP: \textit{Spatial Transform Pyramid}; Cell size 0.5: the cell size of KPR is 0.5; 2D: front-view auxiliary head.}
\centering
\label{table: ablation}
\scalebox{0.8}{
\begin{tabular}{lll|ll}
\hline
\textbf{VC} & \textbf{STP} & \textbf{KPR} & \textbf{F-Score} & \textbf{X error} \\ \hline
            &              &              & 51.2             & 0.37/0.79                 \\
\checkmark           &              &              & 54.5(+3.3)       & 0.32/0.69                 \\
            & \checkmark            &              & 53.2(+2.0)                 & 0.37/0.79                 \\
            &              & \checkmark            & 53.5(+2.3)                 & 0.37/0.76                 \\
            & \checkmark            & \checkmark            & 55.3(+4.1)                 & 0.36/0.79                 \\
\checkmark           &              & \checkmark            & 56.7(+5.5)                 & 0.31/0.69                 \\
\checkmark           & \checkmark            & \checkmark            & 58.4(+7.2)                 & 0.31/0.66                 \\ \hline
\end{tabular}
}
\end{table}

==> table/table_openlane.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\caption{Comprehensive 3D lane evaluation under different metrics. Our Method outperforms previous 3D methods on the metrics of F-Score.~\\}


\label{table: openLane result}
\scalebox{1.0}{
\begin{tabular}{llllll}
\hline
\textbf{Method} & \textbf{F-Score} & \textbf{X error near} & \textbf{X error far} & \textbf{Z error near} & \textbf{Z error far} \\ \hline
3D-LaneNet\cite{garnett20193d}  & 40.2        & \textbf{0.278} & 0.823          & \textbf{0.159} & 0.714          \\
Gen-LaneNet\cite{guo2020gen} & 29.7        & 0.309          & 0.877          & 0.16           & 0.75           \\
PersFormer\cite{chen2022persformer}  & 47.8        & 0.322          & 0.778          & 0.213          & 0.681          \\
\rowcolor[HTML]{C0C0C0} 
Ours        & \textbf{58.4} & 0.309          & \textbf{0.659} & 0.244          & \textbf{0.631} \\ \hline
\end{tabular}
}


\end{table*}
